Learning Mixed Strategies in Trajectory Games

In multi-agent settings, game theory is a natural framework for describing the strategic interactions of agents whose objectives depend upon one another's behavior. Trajectory games capture these complex effects by design. In competitive settings, this makes them a more faithful interaction model than traditional "predict then plan" approaches. However, current game-theoretic planning methods have important limitations. In this work, we propose two main contributions. First, we introduce an offline training phase which reduces the online computational burden of solving trajectory games. Second, we formulate a lifted game which allows players to optimize multiple candidate trajectories in unison and thereby construct more competitive "mixed" strategies. We validate our approach on a number of experiments using the pursuit-evasion game "tag."

==> problem.tex <==
\section{Problem Formulation}
\label{sec:problem}

We consider a noncooperative motion planning problem, in which  $\numplayers$ agents seek to optimize individual---and especially conflicting---objectives.
These multi-agent decision problems are inherently \emph{dynamic games} played between the agents over time.
In such a game, we presume that the motion of each agent (or player) \player{i} may be described in state space and modeled in discrete time.
That is, at time step $t$, \player{i} has state $\state^i_t \in \xset \subseteq \R^\xdim$, and after applying control input (or action) $\control^i_t \in \uset \subseteq \R^\udim$ the resulting state is given by the relation
\begin{equation}
    \label{eqn:dynamics}
    \state^i_{t+1} = \dynamics^i(\state^i_t, \control^i_t).
\end{equation}
We shall require that the function $\dynamics^i \in C^1$, i.e., that it is continuously differentiable.
Most mechanical processes of interest satisfy this assumption, although contact-rich robotic systems such as dexterous manipulators constitute a notable exception. 

To begin, we shall define agents' motion over a fixed time interval $t \in [\horizon] \equiv \{1, \dots, \horizon\}$; later we shall consider the infinite-horizon setting.
On this interval, denote \player{i}'s trajectory by $\primitive^i = \{(\state^i_t, \control^i_t)\}_{t = 1}^\horizon$, with $\primitive^i \in \primitiveset \equiv (\xset \times \uset)^\horizon$.
To model competition among the agents, we presume that each agent \player{i} seeks to minimize an individual performance metric $\cost^i(\primitive^i, \primitive^{\neg i})$ which depends upon \player{i}'s motion $\primitive^i$ and all other agents' motion $\primitive^{\neg i}$.
In addition, agents may also wish to respect both individual and group constraints, encoding properties such as actuator limits and collision avoidance.
\player{i} thus seeks to solve the problem
\begin{subequations}
\label{eqn:notional_problem}
\begin{align}
    \label{eqn:notional_objective}
    \primitive^{i, *} = \arg \min_{\primitive^i \in \primitiveset}~ &\cost^i(\primitive^i, \primitive^{\neg i})\\
    \label{eqn:notional_indconstraint}
    \mathrm{such~that}~ &\indconstraint^i(\primitive^i) \le 0~\textit{(individual constraint)}\\
    \label{eqn:notional_grpconstraint}
    &\grpconstraint^i(\primitive^i, \primitive^{\neg i}) \le 0~\textit{(group constraint)}.
\end{align}
\end{subequations}
To make this problem concrete, we consider the following recurring example.

\example{
\dfknote{tag example here}
}

Problem \cref{eqn:notional_problem}, repeated for each agent \player{i}, constitute a continuous Nash game, and a set of trajectories $\{\primitive^{i, *}\}_{i = 1}^\numplayers$ which simultaneously solve \cref{eqn:notional_problem} for all agents is called a ``pure'' Nash equilibrium. 
Unfortunately, it is well known that such pure Nash solutions do not always exist.
For example, in the two-player pursuit-evasion example of \cref{fig:front}, we see that there are two natural choices for the evader when trapped in a corner.
Neither constitutes a Nash equilibrium, however, because faced with optimal pursuit in each case, the evader prefers to follow the other trajectory. \dfknote{explain this better}

So-called ``mixed'' Nash solutions do exist as long as the set of possible trajectories, $\primitiveset$, is \emph{finite} \cite{basar1998gametheorybook, nash1950equilibrium}.
In this setting, a mixed solution $\tilde \primitive$ is a probability distribution over $\primitiveset$, denoted $\tilde \primitive \in \Delta (\primitiveset)$, and the pure solution $\primitive$ may be viewed as a Dirac distribution on $\primitiveset$.
Finding a mixed solution amounts to finding a Nash equilibrium of the following game
\begin{subequations}
\label{eqn:notional_problem_mixed}
\begin{align}
    \label{eqn:notional_objective_mixed}
    \tilde{\primitive}^{i, *} = \arg \min_{\tilde{\primitive}^i \in \Delta(\primitiveset)}~ &\E_{\primitive^j \sim \tilde{\primitive}^j, \forall j \in [\numplayers]}\left[\cost^i(\primitive^i, \primitive^{\neg i})\right]\\
    \label{eqn:notional_indconstraint_mixed}
    \mathrm{such~that}~ &\indconstraint^i(\primitive^i) \le 0, \forall \primitive^i \in \supp(\tilde{\primitive}^i)\\
    \label{eqn:notional_grpconstraint_mixed}
    &\grpconstraint^i(\primitive^i, \primitive^{\neg i}) \le 0, \forall \primitive^i \in \supp(\tilde{\primitive}^i), \\
    &\hspace{2cm}~\forall \primitive^{\neg i} \in \prod_{j\ne i} \supp(\tilde{\primitive}^j)\nonumber.
\end{align}
\end{subequations}
In \cref{eqn:notional_problem_mixed}, we have rewritten \player{i}'s objective \cref{eqn:notional_objective} as an expectation taken over all agents' trajectory distributions, and enforced the constraints pointwise on their support.

Unfortunately, the set of each players' trajectories $\primitiveset \equiv (\xset \times \uset)^\horizon$ is uncountably infinite.
This means that, in general, even mixed solutions to the Nash game of \cref{eqn:notional_problem_mixed} may not exist.
In this paper, we propose to learn a sequence of relaxations to \cref{eqn:notional_problem_mixed} which gradually approximate the trajectory planning game.
Each relaxation is guaranteed to have a mixed Nash solution which may be found efficiently.
Crucially, these solutions provide derivative information which allows efficient adjustment of relaxations so that they approximate \cref{eqn:notional_problem_mixed} more and more faithfully over time.





